FastSHAP: Real-Time Shapley Value Estimation

Shapley values are widely used to explain black-box models, but they are costly to calculate because they require many model evaluations. We introduce FastSHAP, a method for estimating Shapley values in a single forward pass using a learned explainer model. FastSHAP amortizes the cost of explaining many inputs via a learning approach inspired by the Shapley value's weighted least squares characterization, and it can be trained using standard stochastic gradient optimization. We compare FastSHAP to existing estimation approaches, revealing that it generates high-quality explanations with orders of magnitude speedup.

==> tables/cifar10_auc.tex <==
\begin{table}
\caption{\small{\textbf{Area under the inclusion and exclusion evaluation curves for CIFAR-10.} Area under the curve (AUC) values were obtained from the curves depicting the degradation or improvement in top 1 accuracy as an increasing percentage of the pixels estimated to be important are either excluded or included from the set of 1000 images. For the exclusion AUCs smaller values are better, while for the inclusion AUCs larger values are better.}}
\label{tab:cifar10_auc}
\vskip 0.2in
\begin{center}
\begin{small}
\begin{tabular}{lcccc}
\toprule
 & Exclusion AUC & Inclusion AUC \\
\midrule
FastSHAP & \textbf{0.42(0.41, 0.43)} & 0.78(0.77, 0.79)\\
KernelSHAP & 0.64(0.63, 0.65) & 0.78(0.77, 0.79)\\
KernelSHAP(+) & 0.54(0.53, 0.55) & \textbf{0.86(0.85, 0.87)}\\
GradCAM & 0.52(0.51, 0.54) & 0.76(0.75, 0.77)\\
Integrated Gradients & 0.55(0.54, 0.57) & 0.75(0.74, 0.76)\\
SmoothGrad & 0.70(0.69, 0.72) & 0.72(0.71, 0.73)\\
DeepSHAP & 0.65(0.64, 0.67) & 0.79(0.78, 0.80)\\
\bottomrule
\end{tabular}
\end{small}
\end{center}
% \vskip -0.2in
\end{table}

==> tables/imagenette_auc.tex <==
\begin{table}
\caption{\small{\textbf{Area under the inclusion and exclusion evaluation curves for Imagenette.} Area under the curve (AUC) values were obtained from the curves depicting the degradation or improvement in top 1 accuracy as an increasing percentage of the pixels estimated to be important are either excluded or included from the set of 1000 images. For the exclusion AUCs smaller values are better, while for the inclusion AUCs larger values are better.}}
\label{tab:imagenette_auc}
\vskip 0.2in
\begin{center}
\begin{small}
\begin{tabular}{lcccc}
\toprule
 & Exclusion AUC & Inclusion AUC \\
\midrule
FastSHAP & \textbf{0.51(0.49, 0.52)} & 0.79(0.78, 0.80) \\
KernelSHAP & 0.68(0.67, 0.70) & 0.77(0.75, 0.78) \\
KernelSHAP(+) & 0.61(0.60, 0.63) & \textbf{0.82(0.81, 0.83)} \\
GradCAM & 0.52(0.50, 0.53) & 0.74(0.73, 0.76) \\
Integrated Gradients & 0.65(0.64, 0.66) & 0.73(0.72, 0.75) \\
SmoothGrad & 0.72(0.70, 0.73) & 0.73(0.72, 0.74) \\
DeepSHAP & 0.69(0.68, 0.71) & 0.74(0.73, 0.75) \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
% \vskip -0.2in
\end{table}

==> tables/imagenette_times.tex <==
\begin{table}
\caption{\small{\textbf{.} .}}
\label{tab:imagenette_time}
\vskip 0.2in
\begin{center}
\begin{small}
\begin{tabular}{lcccc}
\toprule
 & Training Time (mins) & Explaining Time (mins) \\
\midrule
FastSHAP &  & 0.04 \\
KernelSHAP &  & 1089.50 \\
KernelSHAP(+) &  & 586.12 \\
GradCAM &  & 1.18 \\
Integrated Gradients &  & 0.73 \\
SmoothGrad &  & 1.17 \\
DeepSHAP &  & 3.39 \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
% \vskip -0.2in
\end{table}
